Translation Deserves Better: Analyzing Translation Artifacts in Cross-lingual Visual Question Answering

Building a reliable visual question answering~(VQA) system across different languages is a challenging problem, primarily due to the lack of abundant samples for training. To address this challenge, recent studies have employed machine translation systems for the cross-lingual VQA task. This involves translating the evaluation samples into a source language (usually English) and using monolingual models (i.e., translate-test). However, our analysis reveals that translated texts contain unique characteristics distinct from human-written ones, referred to as translation artifacts. We find that these artifacts can significantly affect the models, confirmed by extensive experiments across diverse models, languages, and translation processes. In light of this, we present a simple data augmentation strategy that can alleviate the adverse impacts of translation artifacts.

==> acl_latex <==

\begin{thebibliography}{75}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Agrawal et~al.(2015)Agrawal, Lu, Antol, Mitchell, Zitnick, Parikh, and Batra}]{Agrawal2015VQAVQ}
Aishwarya Agrawal, Jiasen Lu, Stanislaw Antol, Margaret Mitchell, C.~Lawrence Zitnick, Devi Parikh, and Dhruv Batra. 2015.
\newblock \href {https://api.semanticscholar.org/CorpusID:3180429} {Vqa: Visual question answering}.
\newblock \emph{International Journal of Computer Vision}, 123:4 -- 31.

\bibitem[{Artetxe et~al.(2023)Artetxe, Goswami, Bhosale, Fan, and Zettlemoyer}]{artetxe2023revisiting}
Mikel Artetxe, Vedanuj Goswami, Shruti Bhosale, Angela Fan, and Luke Zettlemoyer. 2023.
\newblock Revisiting machine translation for cross-lingual classification.
\newblock \emph{arXiv preprint arXiv:2305.14240}.

\bibitem[{Artetxe et~al.(2020)Artetxe, Labaka, and Agirre}]{artetxe-etal-2020-translation}
Mikel Artetxe, Gorka Labaka, and Eneko Agirre. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.emnlp-main.618} {Translation artifacts in cross-lingual transfer learning}.
\newblock In \emph{Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 7674--7684.

\bibitem[{Baker(2019)}]{baker2019corpus}
Mona Baker. 2019.
\newblock Corpus linguistics and translation studies*: Implications and applications.
\newblock In \emph{Researching translation in the age of technology and global conflict}, pages 9--24. Routledge.

\bibitem[{Banerjee and Lavie(2005)}]{banerjee-lavie-2005-meteor}
Satanjeev Banerjee and Alon Lavie. 2005.
\newblock \href {https://aclanthology.org/W05-0909} {{METEOR}: An automatic metric for {MT} evaluation with improved correlation with human judgments}.
\newblock In \emph{Proceedings of the {ACL} Workshop on Intrinsic and Extrinsic Evaluation Measures for Machine Translation and/or Summarization}, pages 65--72. Association for Computational Linguistics.

\bibitem[{Bizzoni et~al.(2020)Bizzoni, Juzek, Espa{\~n}a-Bonet, Dutta~Chowdhury, van Genabith, and Teich}]{bizzoni-etal-2020-human}
Yuri Bizzoni, Tom~S Juzek, Cristina Espa{\~n}a-Bonet, Koel Dutta~Chowdhury, Josef van Genabith, and Elke Teich. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.iwslt-1.34} {How human is machine translationese? comparing human and machine translations of text and speech}.
\newblock In \emph{Proceedings of the 17th International Conference on Spoken Language Translation}, pages 280--290.

\bibitem[{Bugliarello et~al.(2022)Bugliarello, Liu, Pfeiffer, Reddy, Elliott, Ponti, and Vuli{\'c}}]{bugliarello-etal-2022-iglue}
Emanuele Bugliarello, Fangyu Liu, Jonas Pfeiffer, Siva Reddy, Desmond Elliott, Edoardo~Maria Ponti, and Ivan Vuli{\'c}. 2022.
\newblock \href {https://proceedings.mlr.press/v162/bugliarello22a.html} {{IGLUE}: A benchmark for transfer learning across modalities, tasks, and languages}.
\newblock In \emph{Proceedings of the 39th International Conference on Machine Learning}, volume 162 of \emph{Proceedings of Machine Learning Research}, pages 2370--2392. PMLR.

\bibitem[{Burchardt(2013)}]{burchardt-2013-multidimensional}
Aljoscha Burchardt. 2013.
\newblock \href {https://aclanthology.org/2013.tc-1.6} {Multidimensional quality metrics: a flexible system for assessing translation quality}.
\newblock In \emph{Proceedings of Translating and the Computer 35}. Aslib.

\bibitem[{Cettolo et~al.(2017)Cettolo, Federico, Bentivogli, Niehues, St{\"u}ker, Sudoh, Yoshino, and Federmann}]{iwslt2017}
Mauro Cettolo, Marcello Federico, Luisa Bentivogli, Jan Niehues, Sebastian St{\"u}ker, Katsuhito Sudoh, Koichiro Yoshino, and Christian Federmann. 2017.
\newblock \href {https://aclanthology.org/2017.iwslt-1.1} {Overview of the {IWSLT} 2017 evaluation campaign}.
\newblock In \emph{Proceedings of the 14th International Conference on Spoken Language Translation}, pages 2--14. International Workshop on Spoken Language Translation.

\bibitem[{Changpinyo et~al.(2023)Changpinyo, Xue, Yarom, Thapliyal, Szpektor, Amelot, Chen, and Soricut}]{maxm}
Beer Changpinyo, Linting Xue, Michal Yarom, Ashish Thapliyal, Idan Szpektor, Julien Amelot, Xi~Chen, and Radu Soricut. 2023.
\newblock \href {https://arxiv.org/abs/2209.05401} {Maxm: Towards multilingual visual question answering}.
\newblock In \emph{Findings of ACL: EMNLP}.

\bibitem[{Chefer et~al.(2021)Chefer, Gur, and Wolf}]{Attentionvisualization}
Hila Chefer, Shir Gur, and Lior Wolf. 2021.
\newblock \href {https://api.semanticscholar.org/CorpusID:232417173} {Generic attention-model explainability for interpreting bi-modal and encoder-decoder transformers}.
\newblock \emph{2021 IEEE/CVF International Conference on Computer Vision (ICCV)}, pages 387--396.

\bibitem[{Chen et~al.(2023)Chen, Hou, Chen, Dai, Shang, Jiang, Liu, Pan, and Wang}]{chen-etal-2023-mclip}
Guanhua Chen, Lu~Hou, Yun Chen, Wenliang Dai, Lifeng Shang, Xin Jiang, Qun Liu, Jia Pan, and Wenping Wang. 2023.
\newblock \href {https://doi.org/10.18653/v1/2023.acl-long.728} {m{CLIP}: Multilingual {CLIP} via cross-lingual transfer}.
\newblock In \emph{Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)}, pages 13028--13043.

\bibitem[{Chen et~al.(2022)Chen, Wang, Changpinyo, Piergiovanni, Padlewski, Salz, Goodman, Grycner, Mustafa, Beyer et~al.}]{pali}
Xi~Chen, Xiao Wang, Soravit Changpinyo, AJ~Piergiovanni, Piotr Padlewski, Daniel Salz, Sebastian Goodman, Adam Grycner, Basil Mustafa, Lucas Beyer, et~al. 2022.
\newblock Pali: A jointly-scaled multilingual language-image model.
\newblock In \emph{The Eleventh International Conference on Learning Representations}.

\bibitem[{Chen et~al.(2020)Chen, Li, Yu, El~Kholy, Ahmed, Gan, Cheng, and Liu}]{chen2019uniter}
Yen-Chun Chen, Linjie Li, Licheng Yu, Ahmed El~Kholy, Faisal Ahmed, Zhe Gan, Yu~Cheng, and Jingjing Liu. 2020.
\newblock Uniter: Universal image-text representation learning.
\newblock In \emph{European conference on computer vision}, pages 104--120.

\bibitem[{Costa-juss{\`a} et~al.(2022)Costa-juss{\`a}, Cross, {\c{C}}elebi, Elbayad, Heafield, Heffernan, Kalbassi, Lam, Licht, Maillard et~al.}]{NLLB}
Marta~R Costa-juss{\`a}, James Cross, Onur {\c{C}}elebi, Maha Elbayad, Kenneth Heafield, Kevin Heffernan, Elahe Kalbassi, Janice Lam, Daniel Licht, Jean Maillard, et~al. 2022.
\newblock No language left behind: Scaling human-centered machine translation.
\newblock \emph{arXiv preprint arXiv:2207.04672}.

\bibitem[{Dai et~al.(2023)Dai, Li, Li, Tiong, Zhao, Wang, Li, Fung, and Hoi}]{instructBLIP}
Wenliang Dai, Junnan Li, Dongxu Li, Anthony Meng~Huat Tiong, Junqi Zhao, Weisheng Wang, Boyang~Albert Li, Pascale Fung, and Steven C.~H. Hoi. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:258615266} {Instructblip: Towards general-purpose vision-language models with instruction tuning}.
\newblock \emph{ArXiv}, abs/2305.06500.

\bibitem[{Edunov et~al.(2020)Edunov, Ott, Ranzato, and Auli}]{edunov-etal-2020-evaluation}
Sergey Edunov, Myle Ott, Marc{'}Aurelio Ranzato, and Michael Auli. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-main.253} {On the evaluation of machine translation systems trained with back-translation}.
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 2836--2846.

\bibitem[{Fan et~al.(2021)Fan, Bhosale, Schwenk, Ma, El-Kishky, Goyal, Baines, Celebi, Wenzek, Chaudhary et~al.}]{M2M-100}
Angela Fan, Shruti Bhosale, Holger Schwenk, Zhiyi Ma, Ahmed El-Kishky, Siddharth Goyal, Mandeep Baines, Onur Celebi, Guillaume Wenzek, Vishrav Chaudhary, et~al. 2021.
\newblock Beyond english-centric multilingual machine translation.
\newblock \emph{Journal of Machine Learning Research}, 22(107):1--48.

\bibitem[{Gao et~al.(2023)Gao, Han, Zhang, Lin, Geng, Zhou, Zhang, Lu, He, Yue et~al.}]{llama_adapter_v2}
Peng Gao, Jiaming Han, Renrui Zhang, Ziyi Lin, Shijie Geng, Aojun Zhou, Wei Zhang, Pan Lu, Conghui He, Xiangyu Yue, et~al. 2023.
\newblock Llama-adapter v2: Parameter-efficient visual instruction model.
\newblock \emph{arXiv preprint arXiv:2304.15010}.

\bibitem[{Geigle et~al.(2023)Geigle, Jain, Timofte, and Glava{\v{s}}}]{geigle2023mblip}
Gregor Geigle, Abhay Jain, Radu Timofte, and Goran Glava{\v{s}}. 2023.
\newblock mblip: Efficient bootstrapping of multilingual vision-llms.
\newblock \emph{arXiv preprint arXiv:2307.06930}.

\bibitem[{Gellerstam(1986)}]{Gellerstam1986TranslationeseIS}
Martin Gellerstam. 1986.
\newblock Translationese in swedish novels translated from english.
\newblock \emph{Translation studies in Scandinavia}, 1:88--95.

\bibitem[{Goyal et~al.(2016)Goyal, Khot, Summers-Stay, Batra, and Parikh}]{Goyal2016MakingTV}
Yash Goyal, Tejas Khot, Douglas Summers-Stay, Dhruv Batra, and Devi Parikh. 2016.
\newblock \href {https://api.semanticscholar.org/CorpusID:8081284} {Making the v in vqa matter: Elevating the role of image understanding in visual question answering}.
\newblock \emph{International Journal of Computer Vision}, 127:398 -- 414.

\bibitem[{He et~al.(2016)He, Zhang, Ren, and Sun}]{resnet}
Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun. 2016.
\newblock Deep residual learning for image recognition.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 770--778.

\bibitem[{Heusel et~al.(2017)Heusel, Ramsauer, Unterthiner, Nessler, and Hochreiter}]{fid}
Martin Heusel, Hubert Ramsauer, Thomas Unterthiner, Bernhard Nessler, and Sepp Hochreiter. 2017.
\newblock \href {https://proceedings.neurips.cc/paper_files/paper/2017/file/8a1d694707eb0fefe65871369074926d-Paper.pdf} {Gans trained by a two time-scale update rule converge to a local nash equilibrium}.
\newblock In \emph{Advances in Neural Information Processing Systems}, volume~30. Curran Associates, Inc.

\bibitem[{Holtzman et~al.(2019)Holtzman, Buys, Du, Forbes, and Choi}]{holtzman2019curious}
Ari Holtzman, Jan Buys, Li~Du, Maxwell Forbes, and Yejin Choi. 2019.
\newblock The curious case of neural text degeneration.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Hudson and Manning(2019)}]{hudson2019gqa}
Drew~A Hudson and Christopher~D Manning. 2019.
\newblock Gqa: A new dataset for real-world visual reasoning and compositional question answering.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 6700--6709.

\bibitem[{Jain et~al.(2021)Jain, Guo, Srinivasan, Chen, Kudugunta, Jia, Yang, and Baldridge}]{jain-etal-2021-mural-multimodal}
Aashi Jain, Mandy Guo, Krishna Srinivasan, Ting Chen, Sneha Kudugunta, Chao Jia, Yinfei Yang, and Jason Baldridge. 2021.
\newblock \href {https://doi.org/10.18653/v1/2021.findings-emnlp.293} {{MURAL}: Multimodal, multitask representations across languages}.
\newblock In \emph{Findings of the Association for Computational Linguistics: EMNLP 2021}, pages 3449--3463.

\bibitem[{Krishna et~al.(2017)Krishna, Zhu, Groth, Johnson, Hata, Kravitz, Chen, Kalantidis, Li, Shamma et~al.}]{visualgenome}
Ranjay Krishna, Yuke Zhu, Oliver Groth, Justin Johnson, Kenji Hata, Joshua Kravitz, Stephanie Chen, Yannis Kalantidis, Li-Jia Li, David~A Shamma, et~al. 2017.
\newblock Visual genome: Connecting language and vision using crowdsourced dense image annotations.
\newblock \emph{International journal of computer vision}, 123:32--73.

\bibitem[{Lee et~al.(2022)Lee, Lim, Baek, Roh, and Kim}]{lee-etal-2022-efficient}
Youhan Lee, KyungTae Lim, Woonhyuk Baek, Byungseok Roh, and Saehoon Kim. 2022.
\newblock \href {https://aclanthology.org/2022.coling-1.504} {Efficient multilingual multi-modal pre-training through triple contrastive loss}.
\newblock In \emph{Proceedings of the 29th International Conference on Computational Linguistics}, pages 5730--5744.

\bibitem[{Lembersky et~al.(2012)Lembersky, Ordan, and Wintner}]{lembersky2012adapting}
Gennadi Lembersky, Noam Ordan, and Shuly Wintner. 2012.
\newblock Adapting translation models to translationese improves smt.
\newblock In \emph{Proceedings of the 13th Conference of the European Chapter of the Association for Computational Linguistics}, pages 255--265.

\bibitem[{Li et~al.(2023{\natexlab{a}})Li, Li, Savarese, and Hoi}]{BLIP2}
Junnan Li, Dongxu Li, Silvio Savarese, and Steven Hoi. 2023{\natexlab{a}}.
\newblock {BLIP-2:} bootstrapping language-image pre-training with frozen image encoders and large language models.
\newblock \emph{Proceedings of the International Conference on Machine Learning (ICML)}.

\bibitem[{Li et~al.(2020)Li, Yatskar, Yin, Hsieh, and Chang}]{li2019visualbert}
Liunian~Harold Li, Mark Yatskar, Da~Yin, Cho-Jui Hsieh, and Kai-Wei Chang. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-main.469} {What does {BERT} with vision look at?}
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 5265--5275.

\bibitem[{Li et~al.(2023{\natexlab{b}})Li, Fan, Chen, Zhang, Huang, and Wei}]{li-etal-2023-unifying}
Zejun Li, Zhihao Fan, Jingjing Chen, Qi~Zhang, Xuanjing Huang, and Zhongyu Wei. 2023{\natexlab{b}}.
\newblock \href {https://doi.org/10.18653/v1/2023.acl-long.327} {Unifying cross-lingual and cross-modal modeling towards weakly supervised multilingual vision-language pre-training}.
\newblock In \emph{Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)}, pages 5939--5958.

\bibitem[{Lin et~al.(2014)Lin, Maire, Belongie, Hays, Perona, Ramanan, Doll{\'a}r, and Zitnick}]{lin2014microsoft}
Tsung-Yi Lin, Michael Maire, Serge Belongie, James Hays, Pietro Perona, Deva Ramanan, Piotr Doll{\'a}r, and C~Lawrence Zitnick. 2014.
\newblock Microsoft coco: Common objects in context.
\newblock In \emph{Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part V 13}, pages 740--755. Springer.

\bibitem[{Liu et~al.(2023{\natexlab{a}})Liu, Pfeiffer, Korhonen, Vuli{\'c}, and Gurevych}]{liu2023delving}
Chen Liu, Jonas Pfeiffer, Anna Korhonen, Ivan Vuli{\'c}, and Iryna Gurevych. 2023{\natexlab{a}}.
\newblock Delving deeper into cross-lingual visual question answering.
\newblock In \emph{Findings of the Association for Computational Linguistics: EACL 2023}, pages 2408--2423.

\bibitem[{Liu et~al.(2023{\natexlab{b}})Liu, Li, Wu, and Lee}]{llava}
Haotian Liu, Chunyuan Li, Qingyang Wu, and Yong~Jae Lee. 2023{\natexlab{b}}.
\newblock Visual instruction tuning.
\newblock \emph{arXiv preprint arXiv:2304.08485}.

\bibitem[{Liu et~al.(2019)Liu, Ott, Goyal, Du, Joshi, Chen, Levy, Lewis, Zettlemoyer, and Stoyanov}]{liu2019roberta}
Yinhan Liu, Myle Ott, Naman Goyal, Jingfei Du, Mandar Joshi, Danqi Chen, Omer Levy, Mike Lewis, Luke Zettlemoyer, and Veselin Stoyanov. 2019.
\newblock Roberta: A robustly optimized bert pretraining approach.
\newblock \emph{arXiv preprint arXiv:1907.11692}.

\bibitem[{Loshchilov and Hutter(2018)}]{adamw}
Ilya Loshchilov and Frank Hutter. 2018.
\newblock Decoupled weight decay regularization.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Lu et~al.(2019)Lu, Batra, Parikh, and Lee}]{lu2019vilbert}
Jiasen Lu, Dhruv Batra, Devi Parikh, and Stefan Lee. 2019.
\newblock Vilbert: Pretraining task-agnostic visiolinguistic representations for vision-and-language tasks.
\newblock \emph{Advances in neural information processing systems}, 32.

\bibitem[{Mariana(2014)}]{MQM}
Valerie~R Mariana. 2014.
\newblock \emph{The Multidimensional Quality Metric (MQM) framework: A new framework for translation quality assessment}.
\newblock Brigham Young University.

\bibitem[{Marie et~al.(2020)Marie, Rubino, and Fujita}]{marie2020tagged}
Benjamin Marie, Raphael Rubino, and Atsushi Fujita. 2020.
\newblock Tagged back-translation revisited: Why does it really work?
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 5990--5997.

\bibitem[{Marino et~al.(2019)Marino, Rastegari, Farhadi, and Mottaghi}]{Marino2019OKVQAAV}
Kenneth Marino, Mohammad Rastegari, Ali Farhadi, and Roozbeh Mottaghi. 2019.
\newblock \href {https://api.semanticscholar.org/CorpusID:173991173} {Ok-vqa: A visual question answering benchmark requiring external knowledge}.
\newblock \emph{2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, pages 3190--3199.

\bibitem[{Moghe et~al.(2023)Moghe, Sherborne, Steedman, and Birch}]{moghe-etal-2023-extrinsic}
Nikita Moghe, Tom Sherborne, Mark Steedman, and Alexandra Birch. 2023.
\newblock \href {https://doi.org/10.18653/v1/2023.acl-long.730} {Extrinsic evaluation of machine translation metrics}.
\newblock In \emph{Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)}, pages 13060--13078.

\bibitem[{Ni et~al.(2022)Ni, Jin, Freitag, Sachan, and Sch{\"o}lkopf}]{original_or_transalted}
Jingwei Ni, Zhijing Jin, Markus Freitag, Mrinmaya Sachan, and Bernhard Sch{\"o}lkopf. 2022.
\newblock \href {https://doi.org/10.18653/v1/2022.naacl-main.389} {Original or translated? a causal analysis of the impact of translationese on machine translation performance}.
\newblock In \emph{Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies}, pages 5303--5320.

\bibitem[{Ni et~al.(2021)Ni, Huang, Su, Cui, Bharti, Wang, Zhang, and Duan}]{m3p}
Minheng Ni, Haoyang Huang, Lin Su, Edward Cui, Taroon Bharti, Lijuan Wang, Dongdong Zhang, and Nan Duan. 2021.
\newblock M3p: Learning universal representations via multitask multilingual multimodal pre-training.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 3977--3986.

\bibitem[{Nooralahzadeh and Sennrich(2022)}]{Nooralahzadeh2022ImprovingTC}
Farhad Nooralahzadeh and Rico Sennrich. 2022.
\newblock \href {https://api.semanticscholar.org/CorpusID:252111148} {Improving the cross-lingual generalisation in visual question answering}.
\newblock In \emph{AAAI Conference on Artificial Intelligence}.

\bibitem[{OpenAI(2023)}]{OpenAI2023GPT4TR}
OpenAI. 2023.
\newblock \href {https://api.semanticscholar.org/CorpusID:257532815} {Gpt-4 technical report}.
\newblock \emph{ArXiv}, abs/2303.08774.

\bibitem[{Paszke et~al.(2019)Paszke, Gross, Massa, Lerer, Bradbury, Chanan, Killeen, Lin, Gimelshein, Antiga et~al.}]{paszke2019pytorch}
Adam Paszke, Sam Gross, Francisco Massa, Adam Lerer, James Bradbury, Gregory Chanan, Trevor Killeen, Zeming Lin, Natalia Gimelshein, Luca Antiga, et~al. 2019.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock \emph{Advances in neural information processing systems}, 32.

\bibitem[{Pfeiffer et~al.(2022)Pfeiffer, Geigle, Kamath, Steitz, Roth, Vuli{\'c}, and Gurevych}]{xgqa}
Jonas Pfeiffer, Gregor Geigle, Aishwarya Kamath, Jan-Martin Steitz, Stefan Roth, Ivan Vuli{\'c}, and Iryna Gurevych. 2022.
\newblock xgqa: Cross-lingual visual question answering.
\newblock In \emph{Findings of the Association for Computational Linguistics: ACL 2022}, pages 2497--2511.

\bibitem[{Popovi{\'c}(2015)}]{chrf}
Maja Popovi{\'c}. 2015.
\newblock \href {https://doi.org/10.18653/v1/W15-3049} {chr{F}: character n-gram {F}-score for automatic {MT} evaluation}.
\newblock In \emph{Proceedings of the Tenth Workshop on Statistical Machine Translation}, pages 392--395. Association for Computational Linguistics.

\bibitem[{Post(2018)}]{sacrebleu}
Matt Post. 2018.
\newblock \href {https://www.aclweb.org/anthology/W18-6319} {A call for clarity in reporting {BLEU} scores}.
\newblock In \emph{Proceedings of the Third Conference on Machine Translation: Research Papers}, pages 186--191. Association for Computational Linguistics.

\bibitem[{Qiu et~al.(2022)Qiu, Oneaț{\u{a}}, Bugliarello, Frank, and Elliott}]{xuniter}
Chen Qiu, Dan Oneaț{\u{a}}, Emanuele Bugliarello, Stella Frank, and Desmond Elliott. 2022.
\newblock Multilingual multimodal learning with machine translated text.
\newblock In \emph{Findings of the Association for Computational Linguistics: EMNLP 2022}, pages 4178--4193.

\bibitem[{Radford et~al.(2021)Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin, Clark et~al.}]{CLIP}
Alec Radford, Jong~Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, et~al. 2021.
\newblock Learning transferable visual models from natural language supervision.
\newblock In \emph{International conference on machine learning}, pages 8748--8763. PMLR.

\bibitem[{Riley et~al.(2020)Riley, Caswell, Freitag, and Grangier}]{riley-etal-2020-translationese}
Parker Riley, Isaac Caswell, Markus Freitag, and David Grangier. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-main.691} {Translationese as a language in {``}multilingual{''} {NMT}}.
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 7737--7746.

\bibitem[{Schwenk et~al.(2022)Schwenk, Khandelwal, Clark, Marino, and Mottaghi}]{a-okvqa}
Dustin Schwenk, Apoorv Khandelwal, Christopher Clark, Kenneth Marino, and Roozbeh Mottaghi. 2022.
\newblock A-okvqa: A benchmark for visual question answering using world knowledge.
\newblock In \emph{Computer Vision -- ECCV 2022}, pages 146--162. Springer Nature Switzerland.

\bibitem[{Singh et~al.(2022)Singh, Hu, Goswami, Couairon, Galuba, Rohrbach, and Kiela}]{flava}
Amanpreet Singh, Ronghang Hu, Vedanuj Goswami, Guillaume Couairon, Wojciech Galuba, Marcus Rohrbach, and Douwe Kiela. 2022.
\newblock Flava: A foundational language and vision alignment model.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15638--15650.

\bibitem[{Su et~al.(2019)Su, Zhu, Cao, Li, Lu, Wei, and Dai}]{VL_BERT}
Weijie Su, Xizhou Zhu, Yue Cao, Bin Li, Lewei Lu, Furu Wei, and Jifeng Dai. 2019.
\newblock Vl-bert: Pre-training of generic visual-linguistic representations.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Tan and Bansal(2019)}]{LXMERT}
Hao Tan and Mohit Bansal. 2019.
\newblock \href {https://doi.org/10.18653/v1/D19-1514} {{LXMERT}: Learning cross-modality encoder representations from transformers}.
\newblock In \emph{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)}, pages 5100--5111.

\bibitem[{Thapliyal and Soricut(2020)}]{thapliyal-soricut-2020-cross}
Ashish~V. Thapliyal and Radu Soricut. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-main.16} {{C}ross-modal {L}anguage {G}eneration using {P}ivot {S}tabilization for {W}eb-scale {L}anguage {C}overage}.
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 160--170.

\bibitem[{Thapliyal et~al.(2022)Thapliyal, Tuset, Chen, and Soricut}]{crossmodal3600}
Ashish~V Thapliyal, Jordi~Pont Tuset, Xi~Chen, and Radu Soricut. 2022.
\newblock Crossmodal-3600: A massively multilingual multimodal evaluation dataset.
\newblock In \emph{Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing}, pages 715--729.

\bibitem[{Touvron et~al.(2023)Touvron, Lavril, Izacard, Martinet, Lachaux, Lacroix, Rozi{\`e}re, Goyal, Hambro, Azhar et~al.}]{touvron2023llama}
Hugo Touvron, Thibaut Lavril, Gautier Izacard, Xavier Martinet, Marie-Anne Lachaux, Timoth{\'e}e Lacroix, Baptiste Rozi{\`e}re, Naman Goyal, Eric Hambro, Faisal Azhar, et~al. 2023.
\newblock Llama: Open and efficient foundation language models.
\newblock \emph{arXiv preprint arXiv:2302.13971}.

\bibitem[{Vaswani et~al.(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, and Polosukhin}]{vaswani2017attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan~N Gomez, {\L}ukasz Kaiser, and Illia Polosukhin. 2017.
\newblock Attention is all you need.
\newblock \emph{Advances in neural information processing systems}, 30.

\bibitem[{Vedantam et~al.(2015)Vedantam, Lawrence~Zitnick, and Parikh}]{vedantam2015cider}
Ramakrishna Vedantam, C~Lawrence~Zitnick, and Devi Parikh. 2015.
\newblock Cider: Consensus-based image description evaluation.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 4566--4575.

\bibitem[{Volansky et~al.(2015)Volansky, Ordan, and Wintner}]{volansky2015features}
Vered Volansky, Noam Ordan, and Shuly Wintner. 2015.
\newblock On the features of translationese.
\newblock \emph{Digital Scholarship in the Humanities}, 30(1):98--118.

\bibitem[{Wang et~al.(2022)Wang, Meng, Zhang, Liang, Xu, Li, and Zhou}]{CLS_translationese}
Jiaan Wang, Fandong Meng, Tingyi Zhang, Yunlong Liang, Jiarong Xu, Zhixu Li, and Jie Zhou. 2022.
\newblock Understanding translationese in cross-lingual summarization.
\newblock \emph{arXiv preprint arXiv:2212.07220}.

\bibitem[{Wang et~al.(2021)Wang, Tu, Tan, Shi, Sun, and Liu}]{wang-etal-2021-language-coverage}
Shuo Wang, Zhaopeng Tu, Zhixing Tan, Shuming Shi, Maosong Sun, and Yang Liu. 2021.
\newblock \href {https://doi.org/10.18653/v1/2021.findings-acl.422} {On the language coverage bias for neural machine translation}.
\newblock In \emph{Findings of the Association for Computational Linguistics: ACL-IJCNLP 2021}, pages 4778--4790.

\bibitem[{Wolf et~al.(2020)Wolf, Debut, Sanh, Chaumond, Delangue, Moi, Cistac, Rault, Louf, Funtowicz, Davison, Shleifer, von Platen, Ma, Jernite, Plu, Xu, Scao, Gugger, Drame, Lhoest, and Rush}]{wolf-etal-2020-transformers}
Thomas Wolf, Lysandre Debut, Victor Sanh, Julien Chaumond, Clement Delangue, Anthony Moi, Pierric Cistac, Tim Rault, Rémi Louf, Morgan Funtowicz, Joe Davison, Sam Shleifer, Patrick von Platen, Clara Ma, Yacine Jernite, Julien Plu, Canwen Xu, Teven~Le Scao, Sylvain Gugger, Mariama Drame, Quentin Lhoest, and Alexander~M. Rush. 2020.
\newblock \href {https://www.aclweb.org/anthology/2020.emnlp-demos.6} {Transformers: State-of-the-art natural language processing}.
\newblock In \emph{Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: System Demonstrations}, pages 38--45, Online. Association for Computational Linguistics.

\bibitem[{Xie et~al.(2017)Xie, Girshick, Doll{\'a}r, Tu, and He}]{resnext}
Saining Xie, Ross Girshick, Piotr Doll{\'a}r, Zhuowen Tu, and Kaiming He. 2017.
\newblock Aggregated residual transformations for deep neural networks.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 1492--1500.

\bibitem[{Yang et~al.(2021)Yang, Chen, Zhou, and Li}]{yang2021enhancing}
Huiyun Yang, Huadong Chen, Hao Zhou, and Lei Li. 2021.
\newblock Enhancing cross-lingual transfer by manifold mixup.
\newblock In \emph{International Conference on Learning Representations}.

\bibitem[{Yao and Wan(2020)}]{yao-wan-2020-multimodal}
Shaowei Yao and Xiaojun Wan. 2020.
\newblock \href {https://doi.org/10.18653/v1/2020.acl-main.400} {Multimodal transformer for multimodal machine translation}.
\newblock In \emph{Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}, pages 4346--4350.

\bibitem[{Yu et~al.(2022)Yu, Sun, Zhang, and Jiang}]{yu-etal-2022-translate}
Sicheng Yu, Qianru Sun, Hao Zhang, and Jing Jiang. 2022.
\newblock \href {https://doi.org/10.18653/v1/2022.acl-short.40} {Translate-train embracing translationese artifacts}.
\newblock In \emph{Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)}, pages 362--370.

\bibitem[{Zeng et~al.(2022)Zeng, Zhou, Luo, and Zhang}]{Zeng2022CrossViewLM}
Yan Zeng, Wangchunshu Zhou, Ao~Luo, and Xinsong Zhang. 2022.
\newblock \href {https://api.semanticscholar.org/CorpusID:249240598} {Cross-view language modeling: Towards unified cross-lingual cross-modal pre-training}.
\newblock In \emph{Annual Meeting of the Association for Computational Linguistics}.

\bibitem[{Zhang and Toral(2019)}]{zhang-toral-2019-effect}
Mike Zhang and Antonio Toral. 2019.
\newblock \href {https://doi.org/10.18653/v1/W19-5208} {The effect of translationese in machine translation test sets}.
\newblock In \emph{Proceedings of the Fourth Conference on Machine Translation (Volume 1: Research Papers)}, pages 73--81.

\bibitem[{Zhou et~al.(2021)Zhou, Zhou, Wang, Cheng, Li, Yu, and Liu}]{uc2}
Mingyang Zhou, Luowei Zhou, Shuohang Wang, Yu~Cheng, Linjie Li, Zhou Yu, and Jingjing Liu. 2021.
\newblock Uc2: Universal cross-lingual cross-modal vision-and-language pre-training.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 4155--4165.

\bibitem[{Zhu et~al.(2015)Zhu, Groth, Bernstein, and Fei-Fei}]{Zhu2015Visual7WGQ}
Yuke Zhu, Oliver Groth, Michael~S. Bernstein, and Li~Fei-Fei. 2015.
\newblock \href {https://api.semanticscholar.org/CorpusID:5714907} {Visual7w: Grounded question answering in images}.
\newblock \emph{2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, pages 4995--5004.

\end{thebibliography}



==> resources/table/cross_full.tex <==
\begin{table*}[t!]
\tiny
\centering
\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{clc|ccccccccc}
    \bottomrule
    \textbf{Models} & \multicolumn{1}{c}{\textbf{RT?}} & \multicolumn{1}{c}{en} & en$^*$ & bn & de & id & ko & pt & ru & zh & \textbf{avg.} \\ \noalign{\vskip 0.15ex}
    \hline    
    \multicolumn{12}{c}{\textit{\textbf{Zero-Shot}}} \\ \hline
    MUNITER &  & \textbf{57.33} & 50.14 & 14.25 & 30.59 & 17.69 & 20.09 & 23.37 & 20.03 & 19.41 & 20.78 \\
    XUNITER &  & 56.98 & 49.90 & 16.74 & 37.97 & 37.62 & 22.59 & 25.72 & 24.56 & 28.88 & 27.73 \\
    UC$^2$ &  & 56.85 & \textbf{50.22} & \textbf{24.46} & \textbf{48.43} & 36.87 & 32.86 & \textbf{36.28} & \textbf{40.17} & \textbf{38.17} & \textbf{36.75} \\
    M$^3$P &  & 54.45 & 49.29 & 22.75 & 37.96 & \textbf{39.39} & \textbf{34.02} & 34.05 & 31.88 & 35.84 & 33.70 \\
    \hline
    \multicolumn{12}{c}{\textit{\textbf{Translate-Train}}} \\ \hline
    MUNITER &  & \textbf{57.33} & 50.14 & 48.82 & 54.72 & 52.50 & 51.08 & 54.29 & \textbf{54.09} & 51.20 & 52.39 \\
    XUNITER &  & 56.98 & 49.90 & 50.81 & 54.01 & \textbf{53.29} & 51.51 & \textbf{54.72} & 53.87 & 50.26 & 52.64 \\
    UC$^2$ &  & 56.85 & \textbf{50.22} & \textbf{50.82} & \textbf{55.11} & 52.67 & \textbf{51.92} & 54.58 & 53.85 & \textbf{51.94} & \textbf{52.98} \\
    M$^3$P &  & 54.45 & 49.29 & 47.48 & 50.60 & 46.43 & 46.73 & 50.80 & 50.29 & 45.69 & 48.29 \\
    \hline
    \multicolumn{12}{c}{\textit{\textbf{Translate-Test}}} \\ \hline
    \multirow{2}{*}{MUNITER} &  & 57.33 & 50.14 & 50.67 & 54.09 & 52.54 & 50.67 & 54.21 & 49.69 & 49.57 & 51.63 \\
     & \multicolumn{1}{c}{\checkmark} & 55.70 &  52.75 & 52.34 & 55.66 & 53.48 & 53.36 & 54.72 & 53.98 & 52.29 & 53.69 \\
     
    \multirow{2}{*}{XUNITER} &  & 56.98 & 49.90 & 50.76 & 54.63 & 52.37 & 50.52 & 54.24 & 48.91 & 49.94 & 51.62 \\
     & \multicolumn{1}{c}{\checkmark} &55.22 &  52.45  & 52.10 & 54.97 & 52.66 & 52.51 & 54.18 & 52.85 & 52.23 & 53.07\\
     
    \multirow{2}{*}{UC$^2$} &  & 56.85 & 50.22 & 51.34 & 54.01 & 52.35 & 50.75 & 53.81 & 51.93 & 50.04 & 52.03 \\
     & \multicolumn{1}{c}{\checkmark} & 55.12 & 52.44 & 52.35 & 55.10 & 53.29 & 53.07 & 54.17 & 53.36 & 52.73 & 53.44\\
     
     \multirow{2}{*}{M$^3$P} &  & 54.45 & 49.29 & 49.18 & 52.14 & 49.87 & 48.59 & 51.87 & 49.05 & 48.38 & 49.87 \\
     & \multicolumn{1}{c}{\checkmark} & 52.97 & 51.97 & 50.63 & 53.03 & 51.42 & 50.38 & 52.11 & 51.80 & 50.41 & 51.40\\
     
    \multirow{2}{*}{LXMERT} &  & 55.40 & 48.42 & 49.64 & 52.83 & 50.80 & 49.17 & 52.49 & 47.54 & 48.02 & 50.07 \\
     & \multicolumn{1}{c}{\checkmark} & 53.44 & 50.51 & 50.20 & 52.93 & 51.34 & 50.41 & 52.47 & 51.44 & 50.25 & 51.29\\
     
    \multirow{2}{*}{UNITER} &  & 57.47 & 50.11 & 51.74 & 54.52 & 52.79 & 51.27 & 54.56 & 52.27 & 50.33 & 52.50 \\
     & \multicolumn{1}{c}{\checkmark} & 55.92 & 52.90 & 52.32 & 55.53 & 53.67 & 52.93 & 54.66 & 53.56 & 52.60 & 53.61\\
     
    \multirow{2}{*}{VILBERT} &   & 56.72 & 50.10 & 50.84 & 54.10 & 52.27 & 50.73 & 53.98 & 49.91 & 49.92 & 51.68 \\
     & \multicolumn{1}{c}{\checkmark} & 55.22 & 52.52 & 52.23 & 54.85 & 53.43 & 52.75 & 54.26 & 53.69 & 52.22 & 53.35\\
     
    \multirow{2}{*}{VisualBERT} &   & 55.17 & 48.66 & 49.43 & 52.58 & 50.34 & 48.66 & 52.72 & 50.50 & 48.89 & 50.45 \\
     & \multicolumn{1}{c}{\checkmark} & 53.51 & 50.91 & 50.57 & 53.10 & 51.17 & 50.45 & 52.59 & 51.47 & 50.97 & 51.47\\
     
    \multirow{2}{*}{VL-BERT} &   & 57.79 & 50.32 & 51.22 & 54.47 & 52.62 & 50.94 & 54.79 & 51.17 & 50.02 & 52.18 \\
     & \multicolumn{1}{c}{\checkmark} & 55.61 & 52.79 & 52.38 & 55.27 & 53.43 & 52.58 & 54.63 & 53.32 & 52.31 & 53.42\\
     
    \multirow{2}{*}{BLIP-2} &  & 58.05 & 52.10 & 52.03 & 54.70 & 52.99 & 51.57 & 54.91 & 52.36 & 51.22 & 52.83 \\
     & \multicolumn{1}{c}{\checkmark} & 56.11 & 54.76 & 53.18 & 55.70 & 53.98 & 53.51 & 55.11 & 54.25 & 53.31 & 54.15\\
     
    \multirow{2}{*}{InstructBLIP} &  & 57.85 & 52.26 & 51.80 & 54.91 & 53.01 & 51.29 & 54.85 & 53.16 & 51.34 & 52.91 \\
     & \multicolumn{1}{c}{\checkmark} & 55.84 & 54.62 & 53.04 & 55.06 & 53.82 & 53.17 & 54.32 & 54.08 & 53.18 & 53.81\\
     
    \multirow{2}{*}{FLAVA} &  & \textbf{58.84} & 52.91 & 53.47 & 56.26 & 54.11 & 52.85 & 55.84 & 53.64 & 52.18 & 54.05 \\
     & \multicolumn{1}{c}{\checkmark} & 56.87 & \textbf{55.07} & \textbf{53.94} & \textbf{56.35} & \textbf{54.99} & \textbf{54.51} & \textbf{55.96} & \textbf{55.61} & \textbf{53.82} & \textbf{55.03}\\ 
     \toprule
    \end{tabular}
\end{adjustbox}
\caption{Accuracy of models on different cross-lingual approaches. For \textit{Translate-Test}, we use an evaluation set released by \citet{bugliarello-etal-2022-iglue} which is translated with Google Machine Translation~(GMT). en$^*$ denotes the RT-translated English evaluation set. 
The highest scores within each cross-lingual transfer approach in each column are highlighted in \textbf{bold}.
}
\label{tab:appendix_cross_main}
\end{table*}


